Modeling Friendship Networks among Agents with Personality Traits

Using network analysis, psychologists have already found the nontrivial correlation between personality and social network structure. Despite the large amount of empirical studies, theoretical analysis and formal models behind such relationship are still lacking. To bridge this gap, we propose a generative model for friendship networks based on personality traits. To the best of our knowledge, this is the first work to explicitly introduce the concept of personality and friendship development into a social network model, with supporting insights from social and personality psychology. We use the model to investigate the effect of two personality traits, extraversion and agreeableness, on network structure. Analytical and simulation results both concur with recent empirical evidence that extraversion and agreeableness are positively correlated with degree. Using this model, we show that the effect of personality on friendship development can amount to the effect of personality on friendship network structure.

==> text/related_work.tex <==
\section{Related Work}
\label{net_related}

There is a plethora of models in generating network, and some for social network specifically. Since it is impossible to review all the previous models, we discuss some canonical models related to our study. 

% Price's model \cite{price1965networks} is one of the first model describing network formation. Price's model is intended to capture the \textit{richer get richer} phenomena, also known as \textit{Matthew effect} \cite{merton1968matthew}, observed in citation network. 
Barab\'{a}si-Albert model (BA model) \cite{barabasi1999emergence} is a highly influential model which takes into the account of network growth. BA model adopts the mechanism of \textit{preferential attachment} to generate networks with power-law degree distribution, which is found in many real world networks \cite{barabasi2009scale}. The simplifications in BA model make it tractable for analysis, which also make them favored by many researchers. However, for modeling networks of friendship, BA model may fail to capture several important characteristics. 

Unlike citation, which is made in certain time point and will not be altered later, friendship is a dynamical process. A friendship can be formed and may dissolve because of various incidents \cite{adams1994integrative}. 
% Neglecting this potential dynamics might lead to biased understanding of social networks. 
On the other hands, in the social world, it is not expected that every individual will behave the same when dealing with friendship. An extravert have more chance to meet others than an introvert, and an agreeable person is more skilled at maintaining relationship. If we ignore these potential dynamics and heterogeneous behaviors, it might be impossible to grasp the complexity of social networks. 

Prior studies address these drawbacks in different ways. Albert and Barab\'{a}si extended the simple BA model to incorporate extra edge addition and edge rewiring \cite{albert2000topology}. Santiago extended the BA model to heterogeneous networks by imposing attachment kernels \cite{santiago2008extended}. Ferretti, Cortelezzi, Yang, Marmorini, and Bianconi studied the generalizations of BA model extensively, including heterogeneous nodes, heterogeneous links, and preferential rewiring \cite{ferretti2012features}. 

The model considered in this study can be viewed as an extension of the generalizations by Ferretti et al. \cite{ferretti2012features}, with a focus on inspiration from the science of personality and friendship. We thus further present what we know about personality and friendship from psychology and other disciplines. 

